Cogito, ergo sum: A Neurobiologically-Inspired Cognition-Memory-Growth System for Code Generation

Large language models based Multi Agent Systems (MAS) have demonstrated promising performance for enhancing the efficiency and accuracy of code generation tasks. However,most existing methods follow a conventional sequence of planning, coding, and debugging,which contradicts the growth-driven nature of human learning process. Additionally,the frequent information interaction between multiple agents inevitably involves high computational costs. In this paper,we propose Cogito,a neurobiologically inspired multi-agent framework to enhance the problem-solving capabilities in code generation tasks with lower cost. Specifically,Cogito adopts a reverse sequence: it first undergoes debugging, then coding,and finally planning. This approach mimics human learning and development,where knowledge is acquired progressively. Accordingly,a hippocampus-like memory module with different functions is designed to work with the pipeline to provide quick retrieval in similar tasks. Through this growth-based learning model,Cogito accumulates knowledge and cognitive skills at each stage,ultimately forming a Super Role an all capable agent to perform the code generation task. Extensive experiments against representative baselines demonstrate the superior performance and efficiency of Cogito. The code is publicly available at https://anonymous.4open.science/r/Cogito-0083.

==> tabs/API-TOKEN.tex <==

\begin{table*}[]
\centering
\renewcommand{\arraystretch}{1.3}
\scalebox{0.81}{
    \begin{tabular}{|cl|cccc|ccc|}
    \cline{1-9}
    \multicolumn{1}{|c|}{\multirow{2}{*}{\textbf{LLM}}}         & \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{Dataset}}} & \multicolumn{4}{c|}{\textbf{Average for Cogito}}                                                                                                 & \multicolumn{2}{c|}{\textbf{\makecell{Average for\\MapCoder}}}                 & \multicolumn{1}{l|}{\textbf{\multirow{2}{*}{\makecell{Token\\Reduction(k)}}}} \\ \cline{3-8} 
    \multicolumn{1}{|c|}{}                             & \multicolumn{1}{c|}{}                         & \multicolumn{1}{c|}{\textbf{\makecell{API Calls}}} & \multicolumn{1}{c|}{\textbf{\makecell{Prompt Tokens (k)}}} & \multicolumn{1}{c|}{\textbf{\makecell{Completion Tokens (k)}}} & \textbf{\makecell{Total Tokens (k)}} & \multicolumn{1}{c|}{\textbf{\makecell{API Calls}}} & \multicolumn{1}{c|}{\textbf{Tokens (k)}} & \multicolumn{1}{c|}{}                    \\ \hline
    \multicolumn{1}{|c|}{\multirow{5}{*}{\rotatebox{90}{\textbf{ChatGPT-3.5}}}} & HumanEval                                     & \multicolumn{1}{c|}{10}        & \multicolumn{1}{c|}{4.95}              & \multicolumn{1}{c|}{1.31}                  & 6.26             & \multicolumn{1}{c|}{17}         & \multicolumn{1}{c|}{10.41}       & \multicolumn{1}{c|}{4.15}                    \\ \cline{2-9} 
    \multicolumn{1}{|c|}{}                             & MBPP                                          & \multicolumn{1}{c|}{9}         & \multicolumn{1}{c|}{3.28}              & \multicolumn{1}{c|}{1.32}                  & 4.60             & \multicolumn{1}{c|}{12}         & \multicolumn{1}{c|}{4.84}       & \multicolumn{1}{c|}{0.24}                    \\ \cline{2-9} 
    \multicolumn{1}{|c|}{}                             & APPS                                          & \multicolumn{1}{c|}{14}        & \multicolumn{1}{c|}{14.74}             & \multicolumn{1}{c|}{2.04}                  & 16.78            & \multicolumn{1}{c|}{21}         & \multicolumn{1}{c|}{26.57}       & \multicolumn{1}{c|}{2.04}                    \\ \cline{2-9} 
    \multicolumn{1}{|c|}{}                             & xCodeEval                                     & \multicolumn{1}{c|}{16}        & \multicolumn{1}{c|}{16.21}             & \multicolumn{1}{c|}{2.69}                  & 18.90            & \multicolumn{1}{c|}{19}         & \multicolumn{1}{c|}{24.10}       & \multicolumn{1}{c|}{7.89}                    \\ \cline{2-9} 
    \multicolumn{1}{|c|}{}                             & CodeContest                                   & \multicolumn{1}{c|}{15}        & \multicolumn{1}{c|}{24.54}             & \multicolumn{1}{c|}{4.02}                  & 28.56            & \multicolumn{1}{c|}{23}         & \multicolumn{1}{c|}{34.95}       & \multicolumn{1}{c|}{6.39}                    \\ \hline
    \multicolumn{1}{|c|}{\multirow{5}{*}{\rotatebox{90}{\textbf{GPT-4}}}}       & HumanEval                                     & \multicolumn{1}{c|}{10}          & \multicolumn{1}{c|}{5.40}                  & \multicolumn{1}{c|}{1.70}                      &7.10                  & \multicolumn{1}{c|}{15}         & \multicolumn{1}{c|}{12.75}       & \multicolumn{1}{c|}{5.65}                    \\ \cline{2-9} 
    \multicolumn{1}{|c|}{}                             & MBPP                                          & \multicolumn{1}{c|}{10}          & \multicolumn{1}{c|}{3.99}                  & \multicolumn{1}{c|}{1.58}                      &5.57                  & \multicolumn{1}{c|}{8}         & \multicolumn{1}{c|}{4.96}       & \multicolumn{1}{c|}{-0.61}                    \\ \cline{2-9} 
    \multicolumn{1}{|c|}{}                             & APPS                                          & \multicolumn{1}{c|}{13}          & \multicolumn{1}{c|}{18.20}                  & \multicolumn{1}{c|}{3.76}                      &21.96                  & \multicolumn{1}{c|}{19}         & \multicolumn{1}{c|}{31.8}       & \multicolumn{1}{c|}{9.84}                    \\ \cline{2-9} 
    \multicolumn{1}{|c|}{}                             & xCodeEval                                     & \multicolumn{1}{c|}{14}          & \multicolumn{1}{c|}{14.01}                  & \multicolumn{1}{c|}{3.91}                      &17.93                  & \multicolumn{1}{c|}{14}         & \multicolumn{1}{c|}{23.45}       & \multicolumn{1}{c|}{5.52}                    \\ \cline{2-9} 
    \multicolumn{1}{|c|}{}                             & CodeContest                                   & \multicolumn{1}{c|}{15}          & \multicolumn{1}{c|}{26.72}                  & \multicolumn{1}{c|}{5.63}                      &32.35                  & \multicolumn{1}{c|}{19}         & \multicolumn{1}{c|}{38.7}       & \multicolumn{1}{c|}{6.35}                    \\ \hline
    \multicolumn{2}{|c|}{\textbf{Average}}                                                                      & \multicolumn{1}{c|}{13}          & \multicolumn{1}{c|}{13.20}                  & \multicolumn{1}{c|}{2.80}                      &16.00                  & \multicolumn{1}{c|}{16.7}         & \multicolumn{1}{c|}{21.25}       & \multicolumn{1}{c|}{5.25}                    \\ \hline
    \end{tabular}
}
\caption{The average number of API calls and the number of tokens used.}
\label{tab:API-Token}
\end{table*}

==> tabs/Overall-Performance.tex <==

\begin{table*}[t]
\centering
\renewcommand{\arraystretch}{1.3}
\scalebox{0.88}{
    \begin{tabular}{|l|l|ccccc|ccc|}
    \hline
    % \toprule[2pt]
    \multirow{3}{*}{\textbf{LLM}}     
        & \multicolumn{1}{c|}{\multirow{3}{*}{\textbf{Approach}}} 
        & \multicolumn{5}{c|}{\textbf{Simple Problems}}                                                                                                                                         & \multicolumn{3}{c|}{\textbf{Contest-Level Problems}}                              
        \\ \cline{3-10} 
                &                           
                    & \multicolumn{1}{c|}{\textbf{HumanEval}} 
                    & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\textbf{HumanEval} \\ \textbf{ET}\end{tabular}} 
                    & \multicolumn{1}{c|}{\textbf{EvalPlus}}
                    & \multicolumn{1}{c|}{\textbf{MBPP}} 
                    & \begin{tabular}[c]{@{}c@{}}\textbf{MBPP} \\ \textbf{ET}\end{tabular} 
                    & \multicolumn{1}{c|}{\textbf{APPS}} 
                    & \multicolumn{1}{c|}{\textbf{xCodeEval}} & \textbf{CodeContest} 
                \\ \hline
                % \\ \midrule[2pt]
    \multicolumn{1}{|c|}{\multirow{9}{*}{\rotatebox{90}{\textbf{ChatGPT-3.5}}}} 
                    & Direct \dag               
                        & \multicolumn{1}{c|}{48.1}      
                        & \multicolumn{1}{c|}{37.2}                                                    
                        & \multicolumn{1}{c|}{66.5}     
                        & \multicolumn{1}{c|}{49.8} 
                        & 37.7                                               
                        & \multicolumn{1}{c|}{8.0}  
                        & \multicolumn{1}{c|}{17.9}      
                        & 5.5         
                    \\ \cline{2-10} 
                     & CoT \dag                  
                        & \multicolumn{1}{c|}{68.9}      
                        & \multicolumn{1}{c|}{55.5}                                                    
                        & \multicolumn{1}{c|}{65.2}     
                        & \multicolumn{1}{c|}{54.5} 
                        & 39.6                                               
                        & \multicolumn{1}{c|}{7.3}  
                        & \multicolumn{1}{c|}{23.6}      
                        & 6.1         
                    \\ \cline{2-10} 
                    & Self-Planning \dag        
                        & \multicolumn{1}{c|}{60.3}      
                        & \multicolumn{1}{c|}{46.2}                                                    
                        & \multicolumn{1}{c|}{-}        
                        & \multicolumn{1}{c|}{55.7} 
                        & 41.9                                               
                        & \multicolumn{1}{c|}{9.3}  
                        & \multicolumn{1}{c|}{18.9}      
                        & 6.1         
                    \\ \cline{2-10} 
                    & Analogical \dag           
                        & \multicolumn{1}{c|}{63.4}      
                        & \multicolumn{1}{c|}{50.6}                                                    
                        & \multicolumn{1}{c|}{59.1}     
                        & \multicolumn{1}{c|}{70.5} 
                        & 46.1                                               
                        & \multicolumn{1}{c|}{6.7}  
                        & \multicolumn{1}{c|}{15.1}      
                        & 7.3         
                    \\ \cline{2-10} 
                    & Reflexion \dag            
                        & \multicolumn{1}{c|}{67.1}      
                        & \multicolumn{1}{c|}{49.4}                                                    
                        & \multicolumn{1}{c|}{62.2}     
                        & \multicolumn{1}{c|}{73.0} 
                        & 47.4                                               
                        & \multicolumn{1}{c|}{-}    
                        & \multicolumn{1}{c|}{-}         
                        & -           
                    \\ \cline{2-10} 
                    & Self-Collaboration \dag   
                        & \multicolumn{1}{c|}{74.4}      
                        & \multicolumn{1}{c|}{56.1}                                                    
                        & \multicolumn{1}{c|}{-}        
                        & \multicolumn{1}{c|}{68.2} 
                        & 49.5                                               
                        & \multicolumn{1}{c|}{-}    
                        & \multicolumn{1}{c|}{-}         
                        & -           
                    \\ \cline{2-10} 
                    & MapCoder \dag             
                        & \multicolumn{1}{c|}{\textcolor{mycolor_3}{\underline{80.5}}}      
                        & \multicolumn{1}{c|}{\textcolor{mycolor_3}{\underline{70.1}}}                                                    
                        & \multicolumn{1}{c|}{\textcolor{mycolor_3}{\underline{71.3}}} 
                        & \multicolumn{1}{c|}{\textcolor{mycolor_3}{\underline{78.3}}} 
                        & \textcolor{mycolor_3}{\underline{54.4}}                                               
                        & \multicolumn{1}{c|}{\textcolor{mycolor_3}{\underline{11.3}}} 
                        & \multicolumn{1}{c|}{\textcolor{mycolor_3}{\underline{27.4}}}      
                        & \textcolor{mycolor_3}{\underline{12.7}}        
                    \\ \cline{2-10} 
                    \multirow{2}{*}{} & \multirow{2}{*}{\textbf{\textcolor{mycolor_2}{Cogito (Ours)}}}  
                        & \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{\makecell{\textcolor{mycolor_2}{90.24} \\ \textcolor{red}{$\uparrow$ 12.1\%}}}}}
                        & \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{\makecell{\textcolor{mycolor_2}{81.71} \\ \textcolor{red}{$\uparrow$ 16.6\%}}}}} 
                        & \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{\makecell{\textcolor{mycolor_2}{82.32} \\ \textcolor{red}{$\uparrow$ 15.5\%}}}}}
                        & \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{\makecell{\textcolor{mycolor_2}{85.14} \\ \textcolor{red}{$\uparrow$ 8.7\%}}}}}
                        & \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{\makecell{\textcolor{mycolor_2}{59.70} \\ \textcolor{red}{$\uparrow$ 9.7\%}}}}}
                        & \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{\makecell{\textcolor{mycolor_2}{18.00} \\ \textcolor{red}{$\uparrow$ 59.29\%}}}}}
                        & \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{\makecell{\textcolor{mycolor_2}{30.19} \\ \textcolor{red}{$\uparrow$ 10.2\%}}}}}
                        & \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{\makecell{\textcolor{mycolor_2}{13.33} \\ \textcolor{red}{$\uparrow$ 5.0\%}}}}}
                    \\  
                        & \multicolumn{1}{c|}{}
                        & \multicolumn{1}{c|}{}
                        & \multicolumn{1}{c|}{}
                        & \multicolumn{1}{c|}{}
                        & \multicolumn{1}{c|}{}
                        & \multicolumn{1}{c|}{}
                        & \multicolumn{1}{c|}{}
                        & \multicolumn{1}{c|}{}
                        & \multicolumn{1}{c|}{}
                    \\ \hline
                    % \\ \midrule[2pt]
    \multicolumn{1}{|c|}{\multirow{8}{*}{\rotatebox{90}{\textbf{GPT-4}}}}   
                    & Direct \dag               
                        & \multicolumn{1}{c|}{80.1}      
                        & \multicolumn{1}{c|}{73.8}                                                    
                        & \multicolumn{1}{c|}{81.7}     
                        & \multicolumn{1}{c|}{81.1} 
                        & 54.7                                               
                        & \multicolumn{1}{c|}{12.7} 
                        & \multicolumn{1}{c|}{32.1}      
                        & 12.1        
                    \\ \cline{2-10}
                    & CoT \dag                  
                        & \multicolumn{1}{c|}{89.0}      
                        & \multicolumn{1}{c|}{61.6}                                                    
                        & \multicolumn{1}{c|}{-}        
                        & \multicolumn{1}{c|}{82.4} 
                        & 56.2                                               
                        & \multicolumn{1}{c|}{11.3} 
                        & \multicolumn{1}{c|}{36.8}      
                        & 5.5         
                    \\ \cline{2-10} 
                    & Self-Planning \dag        
                        & \multicolumn{1}{c|}{85.4}      
                        & \multicolumn{1}{c|}{62.2}                                                    
                        & \multicolumn{1}{c|}{-}        
                        & \multicolumn{1}{c|}{75.8} 
                        & 50.4                                               
                        & \multicolumn{1}{c|}{14.7} 
                        & \multicolumn{1}{c|}{34.0}      
                        & 10.9        
                    \\ \cline{2-10} 
                    & Analogical \dag           
                        & \multicolumn{1}{c|}{66.5}      
                        & \multicolumn{1}{c|}{48.8}                                                    
                        & \multicolumn{1}{c|}{62.2}     
                        & \multicolumn{1}{c|}{58.4} 
                        & 40.3                                               
                        & \multicolumn{1}{c|}{12.0}
                        & \multicolumn{1}{c|}{26.4}      
                        & 10.9        
                    \\ \cline{2-10} 
                    & Reflexion \dag            
                        & \multicolumn{1}{c|}{91.0}      
                        & \multicolumn{1}{c|}{78.7}                                                    
                        & \multicolumn{1}{c|}{81.7}     
                        & \multicolumn{1}{c|}{78.3} 
                        & 51.9                                               
                        & \multicolumn{1}{c|}{-}    
                        & \multicolumn{1}{c|}{-}         
                        & -           
                    \\ \cline{2-10} 
                    & MapCoder \dag             
                        & \multicolumn{1}{c|}{\textcolor{mycolor_3}{\underline{93.9}}}      
                        & \multicolumn{1}{c|}{\textcolor{mycolor_3}{\underline{82.9}}}                                                    
                        & \multicolumn{1}{c|}{\textcolor{mycolor_3}{\underline{83.5}}}     
                        & \multicolumn{1}{c|}{\textcolor{mycolor_3}{\underline{83.1}}} 
                        & \textcolor{mycolor_3}{\underline{57.7}}                                               
                        & \multicolumn{1}{c|}{\textcolor{mycolor_3}{\underline{22}}}   
                        & \multicolumn{1}{c|}{\textcolor{mycolor_3}{\underline{45.3}}}      
                        & \textcolor{mycolor_3}{\underline{28.5}}        
                    \\ \cline{2-10} 
                    \multirow{2}{*}{} & \multirow{2}{*}{\textbf{\textcolor{mycolor_2}{Cogito (Ours)}}}  
                        & \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{\makecell{\textcolor{mycolor_2}{95.73} \\ \textcolor{red}{$\uparrow$ 1.9\%}}}}}
                        & \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{\makecell{\textcolor{mycolor_2}{83.54} \\ \textcolor{red}{$\uparrow$ 0.8\%}}}}} 
                        & \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{\makecell{\textcolor{mycolor_2}{85.37} \\ \textcolor{red}{$\uparrow$ 2.2\%}}}}}
                        & \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{\makecell{\textcolor{mycolor_2}{88.16} \\ \textcolor{red}{$\uparrow$ 6.1\%}}}}}
                        & \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{\makecell{\textcolor{mycolor_2}{66.25} \\ \textcolor{red}{$\uparrow$ 14.8\%}}}}}
                        & \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{\makecell{\textcolor{mycolor_2}{27.30} \\ \textcolor{red}{$\uparrow$ 24.1\%}}}}}
                        & \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{\makecell{\textcolor{mycolor_2}{47.20} \\ \textcolor{red}{$\uparrow$ 4.2\%}}}}}
                        & \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{\makecell{\textcolor{mycolor_2}{29.70} \\ \textcolor{red}{$\uparrow$ 4.2\%}}}}}
                    \\  
                        & \multicolumn{1}{c|}{}
                        & \multicolumn{1}{c|}{}
                        & \multicolumn{1}{c|}{}
                        & \multicolumn{1}{c|}{}
                        & \multicolumn{1}{c|}{}
                        & \multicolumn{1}{c|}{}
                        & \multicolumn{1}{c|}{}
                        & \multicolumn{1}{c|}{}
                        & \multicolumn{1}{c|}{}
                    \\ \hline
                    % \\ \bottomrule[2pt]
    \end{tabular}
}
\caption{Overall performance comparison across various datasets, categorized into \textit{Simple Problems} and \textit{Contest-Level Problems}.  The best performance is highlighted in \textbf{\textcolor{mycolor_2}{blue}}, and the second-best performance is \textcolor{mycolor_3}{\underline{underlined}}. The improvement of \textbf{Cogito} over the previous state-of-the-art (Mapcoder) is highlighted in \textbf{\textcolor{red}{red}}. \dag: Results are publicly disclosed in the paper of MapCoder.}
\label{tab_Overall-Performance}
\end{table*}
